How Many Shots Are Enough for a Quantum Circuit?

Quantum algorithms require repeated circuit executions, known as shots, to estimate output distributions accurately. Determining the minimal number of shots needed to meet a target accuracy is crucial to reduce costs and resource usage, especially on today's noisy and expensive quantum hardware. In this paper, we address the shot optimisation problem in a black-box setting, where no assumptions are made about the structure of the quantum circuit or the noise model of the backend. We introduce IncrementalExecution, a novel online framework that dynamically determines when to stop executing shots based on the principle of point of diminishing returns: the point at which additional shots no longer significantly alter the empirical distribution of a fixed circuit. The framework supports customisable policies for shot management, enabling flexible trade-offs between execution cost and result fidelity within static execution scenarios. We assess our proposal through an extensive experimental evaluation spanning 33,750 framework configurations across 180 unique static quantum circuit-backend combinations, for a total of 7.3M independent experiments. Unlike prior work that relies on problem-specific knowledge or algorithm-dependent assumptions (e.g., variational or adaptive workflows), our approach is applicable to a large set of static circuits and immediately deployable on current quantum cloud platforms.

==> src/conclusions_old.tex <==
\\section{Conclusions and Future Work}
\label{sec:conclusions}

\new{This work addressed the problem of approximating the optimal number of shots for static, non-variational quantum circuits under a fixed shot budget, in a black-box setting that makes no assumptions about circuit structure or backend noise models. We introduced \textsc{IncrementalExecution}, an online framework that reframes shot allocation as an iterative, data-driven stopping problem, and we showed how it can be instantiated through a family of execution policies that trade off cost and statistical fidelity.}

\new{Central to our approach is the concept of the \emph{point of diminishing returns}, which provides an observable stabilisation signal without requiring access to the unknown target distribution. To ground evaluation in a principled baseline, we further introduced the notion of \emph{a posteriori optimality}, which retrospectively identifies the minimal prefix of an execution trace whose empirical distribution matches the best available estimate under the given budget.}

\new{The primary objective of this paper was to establish and validate \textsc{IncrementalExecution} as a general-purpose solution \emph{within the scope of static circuit executions}. Through an extensive empirical evaluation comprising over \new{$7.3$M} experiments across \new{$33{,}750$} policy configurations and \new{180} circuit--backend pairs, our results indicate that:}
\begin{itemize}
    \item \new{\textbf{Policy-driven flexibility for static circuits:} \textsc{IncrementalExecution} can be configured to reach user-specified stability/accuracy targets across the evaluated execution traces, without relying on circuit-specific or backend-specific prior knowledge. This demonstrates that effective shot optimisation can be achieved in a black-box manner when the circuit remains fixed during execution.}

    \item \new{\textbf{Near-optimal online stopping:} Compared to the a posteriori optimal baseline (which assumes access to the full execution history), the overhead incurred by online decision making is typically small, while achieving comparable distributional fidelity under the adopted divergence criterion.}
\end{itemize}

\new{Our evaluation also highlights that there is no universally best configuration: optimal performance depends on properties of the executed circuit and backend (e.g., circuit size and output complexity). This suggests that systematic configuration and meta-optimisation can yield additional gains. As an initial step, we showed that circuit size provides a meaningful signal for guiding such tuning, and we anticipate that richer circuit descriptors could further improve configuration selection.}

\new{Finally, we emphasise that the framework is not only conceptually principled but also practically deployable. Emerging support for session-based execution, reservation models, and hybrid runtimes across quantum cloud platforms makes online stopping strategies increasingly viable in operational settings, where reducing unnecessary shots can translate into tangible savings in time and cost.}

\new{While the IncrementalExecution framework is, in principle, applicable to a broad class of stochastic sampling processes, quantum computing constitutes a domain in which its advantages are particularly pronounced. In this setting, shot budgets translate directly into monetary cost, wall-clock latency, and hardware contention, while oversampling cannot overcome accuracy plateaus induced by noise. As a result, the ability to detect the point of diminishing returns online is uniquely valuable for quantum workloads. In summary, although our methodology is formulated in general statistical terms, it is motivated by, and specifically tailored to, the practical constraints of quantum computing. By abstracting away circuit- and noise-specific assumptions, we offer a broadly applicable solution to a problem widely recognised as timely and important in the quantum computing literature: determining how many shots are sufficient.}

\new{Looking ahead, several directions could further extend the scope and impact of IncrementalExecution:}
\begin{description}
    \item[\new{Beyond fixed-budget baselines.}] \new{In this work, optimality is defined relative to a fixed budget $\mathcal{B}$ via the reference distribution $\hat{P}_\mathcal{B}$. A natural extension is to study a \emph{budget-less} formulation, where the goal is to determine a stopping point without assuming an a priori maximum number of shots. Addressing this setting requires principled criteria for termination under uncertainty (e.g., confidence guarantees or asymptotic stabilisation tests), and we plan to investigate both theoretical and empirical solutions.}

    \item[\new{Integration with complementary execution techniques.}] \new{We currently consider executing a circuit on a single backend. Future work will embed \textsc{IncrementalExecution} into broader quantum workflow optimisations~\cite{bisicchia2024quantum}, including \textit{shot-wise distribution}~\cite{bisicchia2024distributingQCE,bisicchia2023distributing,bisicchia2024distributing}, \textit{circuit cutting}~\cite{tang2021cutqc,bisicchia2024cut,bisicchia2026cut}, and \textit{circuit composition}~\cite{ohkura2022simultaneous,das2019case,bisicchia2025maximizing}. These integrations raise interesting questions about how stabilisation signals compose across distributed and decomposed executions.}

    \item[\new{Learning-based policy design.}] \new{We plan to develop learning-based strategies (e.g., reinforcement learning) to synthesise shot-allocation and stopping policies from data. Such approaches could move beyond static heuristics by conditioning decisions on circuit descriptors, observed stabilisation dynamics, and backend characteristics, learning policies that generalise across circuit families and execution environments.}

    \item[\new{Validation on real quantum hardware.}] \new{While our experiments use realistic noisy simulators, validating the framework on real devices is essential. Real hardware introduces additional factors, including queueing delays, calibration drift, transient failures, and runtime scheduling variability, that may affect both the stopping signal and the realised savings. Empirical evaluation under these conditions is a key next step.}

    \item[\new{Automated hyperparameter tuning and configuration selection.}] \new{Our results show that no single policy configuration is uniformly optimal across all circuit--backend pairs. Future work will therefore explore automated tuning and selection mechanisms, including Bayesian optimisation, evolutionary strategies, and AutoML techniques. By linking circuit properties (e.g., qubit count, depth, output sparsity) to effective hyperparameter settings, we aim to provide practical guidelines and tooling for deploying \textsc{IncrementalExecution} in real-world quantum software workflows.}

    \item[\new{Extension to variational and adaptive workloads.}] \new{A particularly important direction is extending \textsc{IncrementalExecution} to \emph{variational} and other \emph{adaptive} algorithms. Unlike the static setting studied here, these workloads induce non-stationary output distributions because the circuit changes across optimisation iterations. Supporting such settings will require additional mechanisms (e.g., phase-aware stopping rules, change-point detection, or iteration-coupled policies) to disentangle stabilisation from distributional shifts.}
\end{description}

==> src/old_exp.tex <==
\section{Experimental Evaluation}
\label{sec:exp}

This experimental evaluation\footnote{Experimental scripts, raw data and analysis are freely available at: \url{https://github.com/GBisi/quantum-incremental-execution}.} section has a twofold objective: (i) to assess whether there exist configurations capable of achieving the target accuracy while reducing the total number of shots with respect to a fixed budget, and (ii) to provide practical insights and preliminary guidelines for policy fine-tuning as a function of quantum circuit characteristics.

\subsection{Experimental Setup}

We evaluated our framework on a comprehensive benchmark consisting of $140$ unique execution traces, each corresponding to a distinct quantum circuit and backend pair, as introduced in Section~\ref{sec:intro}\footnote{\new{These traces are collected once and used exclusively for offline, retrospective evaluation of different policies under identical noise conditions. In practical deployments, the IncrementalExecution framework would be run online and may terminate well before reaching $\mathcal{B}$, without requiring the full trace.
}}.  Each execution trace provides the complete measurement history, enabling retrospective analysis and ground-truth evaluation of any shot allocation policy under identical noise conditions.

For each trace, the maximum shot budget $\mathcal{B}$ was set to $20,\!000$. We explored the entire policy space described in Section~\ref{sec:policies}, yielding a total of $12,\!474$ unique configurations, each specifying the parameters for stopping criterion, stability enforcement, and shot allocation strategy.

The primary accuracy metric is the Total Variation Distance (TVD) between the empirical distribution $\hat{P}_n$ output by the framework and the empirical reference distribution $\hat{P}_\mathcal{B}$ obtained using all available shots, as per Definition~\ref{def:optimal-shots}. We consider a configuration \emph{successful} if, for all 140 traces, it stops with $\mathrm{TVD}(\hat{P}_n, \hat{P}_\mathcal{B}) \leq \delta$, where $\delta$ is a user-specified tolerance threshold.

\subsection{Configuring for Guaranteed Target Accuracy}

\begin{figure*}[t]
\centering
\subfigure[Successful configurations for $\delta=0.2$.]{\includegraphics[width=0.49\textwidth]{img/confs02.png}}
\hfill
\subfigure[Successful configurations for $\delta=0.3$.]{\includegraphics[width=0.49\textwidth]{img/confs03.png}}
\caption{Average shots saved with respect to the full budget by successful configurations.}
\label{fig:confs}
\end{figure*}

Our first objective is to establish whether \textsc{IncrementalExecution} can be configured to \emph{always} reach the target accuracy, i.e., to output distributions with TVD at most $\delta$ from the full empirical reference \emph{in every execution trace}, while also saving shots compared to the fixed-budget baseline.

To this end, for each target threshold ($\delta=0.2$ and $\delta=0.3$), we filtered the set of $12,\!474$ configurations to retain only those that satisfied the accuracy requirement for all $140$ traces. With $\delta=0.2$, $301$ configurations passed this cut-off filter, and with $\delta=0.3$, $378$ configurations did so.

It is important to note that, even among successful configurations, the average fraction of shots saved with respect to the full budget varies substantially, from approximately $30\%$ to $70\%$ (Fig.~\ref{fig:confs} shows the average shots saved for each successful configuration). This highlights a fundamental property: \emph{no single configuration achieves optimal shot savings across all circuits and scenarios}. Rather, as in the case of hyperparameter selection for classical machine learning models, optimal performance is scenario-dependent, and careful policy and parameter tuning is essential to fully exploit the potential of the framework. Nevertheless, the existence of hundreds of configurations achieving required accuracy across all traces demonstrates the robustness and general applicability of the approach.

\subsection{Guidelines for Policy Fine-Tuning}

As a preliminary step toward practical fine-tuning, we investigated how the best-performing configurations vary as a function of circuit size, an intuitively important factor affecting sampling complexity and convergence dynamics.

We partitioned the dataset into two groups:
\begin{itemize}
    \item \textbf{Small circuits:} circuits counting fewer than $10$ qubits.
    \item \textbf{Large circuits:} circuits counting $10$ or more qubits.
\end{itemize}
This partitioning is motivated by the observation that circuit width typically increases the support size of the output distribution, which, in turn, impacts the number of samples needed for stable estimation.

\paragraph{Outlier Removal.}
To prevent extreme cases from biasing the analysis, we removed outlier traces within each group using the Interquartile Range (IQR) outlier detection methodology. This decision is motivated by three considerations: (i) such traces are extremely rare in practice and may correspond to pathological circuits or anomalous noise behaviour; (ii) their inclusion could skew aggregate performance metrics, reducing the representativeness of validation and test sets; and (iii) this stage of the study is focused on obtaining a robust and interpretable assessment of the framework’s behaviour under typical operating conditions. Indeed, we already demonstrated above that \textsc{IncrementalExecution} can be configured to achieve the target accuracy across \emph{all} 140 traces, including the outliers. Thus, the decision to exclude them here is not a limitation of the framework, but a deliberate step toward more practical, fine-grained analysis of performance trends and configuration strategies under non-pathological settings.

\paragraph{Validation/Test Splitting.}
Within each group, we randomly split the data into an \emph{80\% validation set} and a \emph{20\% test set}. This conventional split ensures sufficient data for robust policy selection while allowing for unbiased performance estimation on held-out circuits. The rationale mirrors standard practice in machine learning, providing statistical support for the conclusions and helping to mitigate overfitting to particular trace characteristics.

\paragraph{Configuration Selection Procedure.}
For each group and each value of $\delta$, we filtered configurations to retain only those that achieved the target TVD threshold on all traces in the \emph{validation set}. Among these, we selected the configuration achieving the highest average shot savings (i.e., the lowest mean shot count) on the validation set, and then evaluated this configuration on the held-out test set.

\subsection{Results and Analysis}

\subsubsection*{Small Circuits ($<$10 qubits), $\delta=0.2$}

The best configuration identified for small circuits and $\delta=0.2$ is as follows:
\begin{itemize}
    \item \texttt{initial\_shots}: $50$
    \item \texttt{shots\_allocation\_policy}: dynamic
    \item \texttt{stopping\_criterion\_threshold}: $0.1$
    \item \texttt{stopping\_criterion\_policy}: dma
    \item \texttt{stability\_k}: $3$
    \item \texttt{dma\_lookback\_window}: $3.0$
    \item \texttt{dma\_window}: $5.0$
    \item \texttt{min\_initial\_iterations}: $5.0$
\end{itemize}
On the test set, this configuration performed an average of $450$ shots per circuit versus $320$ for the optimal a posteriori policy. The mean TVD from the full empirical distribution was $0.09$, well below the $\delta=0.2$ threshold.

\subsubsection*{Large Circuits ($\geq$10 qubits), $\delta=0.2$}

\begin{itemize}
    \item \texttt{initial\_shots}: $250$
    \item \texttt{shots\_allocation\_policy}: dynamic
    \item \texttt{stopping\_criterion\_threshold}: $0.05$
    \item \texttt{stopping\_criterion\_policy}: dma
    \item \texttt{stopping\_dist\_func}: tvd
    \item \texttt{stability\_k}: $5$
    \item \texttt{dma\_lookback\_window}: $2.0$
    \item \texttt{dma\_window}: $3.0$
    \item \texttt{min\_initial\_iterations}: $5.0$
\end{itemize}
This configuration used, on average, $15,\!600$ shots per circuit compared to $15,\!000$ for the a posteriori optimum, with a mean TVD of $0.18$.

\subsubsection*{Small Circuits ($<$10 qubits), $\delta=0.3$}

\begin{itemize}
    \item \texttt{initial\_shots}: $50$
    \item \texttt{shots\_allocation\_policy}: dynamic
    \item \texttt{stopping\_criterion\_threshold}: $0.05$
    \item \texttt{stopping\_criterion\_policy}: delta
    \item \texttt{stopping\_dist\_func}: tvd
    \item \texttt{stability\_k}: $1$
    \item \texttt{dc\_lookback\_window}: $1.0$
    \item \texttt{min\_initial\_iterations}: $3.0$
\end{itemize}
This setting achieved $312$ shots on average (test set), compared to $129$ for the a posteriori optimal policy, with a mean TVD of $0.11$.

\subsubsection*{Large Circuits ($\geq$10 qubits), $\delta=0.3$}

Finally, for large circuits and $\delta=0.3$, the best configuration is:
\begin{itemize}
    \item \texttt{initial\_shots}: $50$
    \item \texttt{shots\_allocation\_policy}: constant, value $250$
    \item \texttt{stopping\_criterion\_threshold}: $0.05$
    \item \texttt{stopping\_criterion\_policy}: dma
    \item \texttt{stopping\_dist\_func}: tvd
    \item \texttt{stability\_k}: $3$
    \item \texttt{dma\_lookback\_window}: $2.0$
    \item \texttt{dma\_window}: $3.0$
    \item \texttt{dma\_alpha}: $0.5$
\end{itemize}
This configuration resulted in an average of $12,\!500$ shots (test set) versus $9,\!900$ for the a posteriori optimum, with a mean TVD of $0.23$.

\subsection{Discussion}

These results illustrate several key points:

\begin{itemize}
    \item \textbf{Flexibility and Generality:} Across both circuit sizes and accuracy thresholds, it is possible to find configurations that guarantee the desired target accuracy \emph{for all} circuits considered, with substantial shot savings over the fixed-budget baseline.
    \item \textbf{No One-Size-Fits-All:} The best-performing configuration varies with circuit size and target accuracy, confirming that practical use of \textsc{IncrementalExecution} should incorporate policy fine-tuning or adaptive policy selection to maximise efficiency.
    \item \textbf{Shot Savings:} For small circuits and moderate accuracy, the shot savings are dramatic (up to $98\%$ compared to the full budget), with minimal loss in fidelity. For larger circuits, shot savings remain significant, though the absolute number of required samples increases, as expected.
    \item \textbf{Framework Overhead:} In all tested scenarios, the framework incurs only a small overhead compared to the a posteriori optimum.
\end{itemize}

\paragraph{Outlook for Fine-Tuning.}
Our preliminary fine-tuning by circuit size demonstrates the importance of customising policy parameters to scenario-specific requirements. In future work, we plan to systematically investigate more sophisticated meta-optimisation and learning-based approaches for online policy selection, leveraging ideas and techniques from classical AutoML and Bayesian optimisation.

\subsection{Summary}

In summary, the experiments demonstrate that \textsc{IncrementalExecution} is capable of robustly and efficiently approximating the optimal shot count in black-box quantum execution. By providing both general-purpose default configurations and supporting targeted fine-tuning, the framework offers a practical solution for balancing execution cost and result fidelity in a wide range of quantum computing applications.

==> src/problem_old.tex <==
\section{The Black-box Sample Optimisation Problem}
\label{sec:problem}

Quantum circuit execution is inherently stochastic, producing measurement outcomes sampled from an unknown output distribution. Estimating this distribution accurately requires repeated sampling -- or \emph{shots} -- but each sample incurs cost and latency, especially on real quantum hardware. The core challenge addressed in this paper is to determine, as efficiently as possible, how many samples (i.e., shots) are sufficient for a given circuit, i.e., the point of diminishing returns.

This section formalises the problem of sample optimisation in a general black-box setting and then incrementally narrows the scope toward practical application in quantum computing. Specifically:
\begin{itemize}
    \item We first define the general problem of estimating an unknown discrete distribution under budget constraints, and introduce an \emph{a posteriori} algorithm to compute the minimal sufficient number of samples.
    \item We then introduce a practical approximation of the point of diminishing returns that can be used in online settings when the true distribution is not accessible.
    \item Finally, we instantiate this problem in the quantum setting, showing how it arises naturally when executing quantum circuits on noisy quantum hardware.
\end{itemize}

\subsection{General Formulation}
\label{sec:problem:general}


In its most general form, the problem addressed in this work can be formulated as follows. Consider a stochastic process that outputs samples drawn from an unknown target distribution $P$ over a finite, discrete outcome space $\mathcal{X}$. Each draw produces a single random, independent sample from $P$, and repeating the process $n$ times yields an empirical distribution $\hat{P}_n$.
%
A distance or divergence metric $\mathcal{D}(\cdot,\cdot)$ is used to quantify the difference between two probability distributions over $\mathcal{X}$. Given a threshold $\delta > 0$ representing the maximum acceptable estimation error and a hard budget $\mathcal{B}$ on the maximum number of available samples, we define the following problem.

\begin{definition}[\textbf{The Black-box Sample Optimisation Problem}]
\label{def:problem}
Given an unknown distribution $P$ over a discrete space $\mathcal{X}$, a divergence metric $\mathcal{D}$, a maximum estimation error threshold $\delta$, and a budget $\mathcal{B} \in \mathbb{N}$, find the smallest positive integer $n^* \leq \mathcal{B}$ such that
\[
n^* = \min \left\{ n \leq \mathcal{B} \mid \mathcal{D}(\hat{P}_n, P) \leq \delta \right\}
\]
where $\hat{P}_n$ is the empirical distribution over the first $n$ samples.
\end{definition}

This general formulation captures the essence of estimating a probability distribution under budget constraints. In practice, however, the true distribution $P$ is unknown and cannot be accessed directly, such as when sampling the ideal output distribution of a quantum circuit.

To address the unknown nature of $P$, we adopt a practical approximation: we define the \emph{reference distribution} $\hat{P}_\mathcal{B}$ as the empirical distribution obtained from all $\mathcal{B}$ available samples. Although $\hat{P}_\mathcal{B}$ is itself an approximation of $P$, it is the best estimate \textit{practically} obtainable given the budget. We then redefine optimality as follows.

% A Posteriori black-box sample optimisation problem
\begin{definition}[\textbf{The A Posteriori Black-box Sample Optimisation Problem}]
\label{def:optimal-shots}
Given an execution history of subsequent $\mathcal{B}$ samples $\{x_1, \dots, x_\mathcal{B}\}$ drawn from an unknown distribution $P$, a divergence metric $\mathcal{D}$, and a target threshold $\delta > 0$, find the \emph{optimal number of samples} $n^* \leq \mathcal{B}$ such that
\[
n^* = \min \left\{ n \leq \mathcal{B} \mid \mathcal{D}(\hat{P}_n, \hat{P}_\mathcal{B}) \leq \delta \right\},
\]
where $\hat{P}_n$ is the empirical distribution over the first $n$ samples and $\hat{P}_\mathcal{B}$ is the empirical distribution over all $\mathcal{B}$ samples.
\end{definition}

This notion of optimality is \textit{a posteriori}, as it relies on having access to all $\mathcal{B}$ samples to compute $\hat{P}_\mathcal{B}$ and assess whether earlier subsets of the execution history were already sufficient to meet the desired estimation error threshold. This definition provides a principled and computable measure of convergence: it identifies the point at which the empirical distribution has stabilised with respect to the best available estimate under the budget. In this sense, $n^*$ captures the earliest point beyond which further execution yields diminishing returns. Notice that, since $\mathcal{D}(\hat{P}_\mathcal{B}, \hat{P}_\mathcal{B})=0$, in the worst case $n^*=\mathcal{B}$.

\paragraph{Optimal Sample Count Algorithm.} We now introduce an \textit{a posteriori} algorithm for computing $n^*$ from an execution history. 


%Algorithm~\ref{alg:aposteriori}\footnote{The pseudocode uses the Python-style dictionary method \texttt{.get(key, default)} to retrieve the current count of a key (outcome) in a dictionary. If the key is not yet present, \texttt{.get()} returns the specified default value (in this case, 0). This avoids key errors during lookup and allows safe incrementation of unseen outcomes.} presents a method to determine the \textit{a posteriori} optimal number of samples, denoted as $n^*$, required to approximate the full empirical distribution $\hat{P}_\mathcal{B}$ within a given divergence threshold $\delta$. This approach assumes access to a full batch of $\mathcal{B}$ measurement outcomes and operates in an \textit{a posteriori} manner -- that is, it uses the complete dataset to evaluate at which point in the sequence of samples the distribution becomes stable.

\begin{algorithm}[H]
\caption{A Posteriori Optimal Sample Count Computation}
\label{alg:aposteriori}
\KwIn{Measurement outcomes $\{x_1, x_2, \dots, x_\mathcal{B}\}$, threshold $\delta$, divergence metric $\mathcal{D}$}
\KwOut{Optimal number of samples $n^* \leq \mathcal{B}$}

// Step 1: Build the reference distribution $\hat{P}_\mathcal{B}$\

\textbf{initialize} $\texttt{count\_B[$k$]} \gets 0$ for all outcomes $k$;

\For{$i \gets 1$ \KwTo $\mathcal{B}$}{
    \texttt{count\_B[$x_i$]} $\gets$ \texttt{count\_B[$x_i$]} $+ 1$\; 
}
\ForEach{key $k$ in \texttt{count\_B}}{
    $\hat{P}_\mathcal{B}[k] \gets$ \texttt{count\_B[$k$]} $/ \mathcal{B}$\;
}

// Step 2: Incrementally build $\hat{P}_n$ and compare with $\hat{P}_\mathcal{B}$\

\textbf{initialize} $\texttt{count\_n[$k$]} \gets 0$ for all outcomes $k$;

\texttt{total\_n} $\gets 0$\;

\For{$n \gets 1$ \KwTo $\mathcal{B}$}{
    \texttt{count\_n[$x_n$]} $\gets$ \texttt{count\_n[$x_n$]} $+ 1$\;
    \texttt{total\_n} $\gets$ \texttt{total\_n} $+ 1$\;
    
    \ForEach{key $k$ in \texttt{count\_B}}{
        $f \gets$ \texttt{count\_n.get[$k$]}\;
        $\hat{P}_n[k] \gets f / \texttt{total\_n}$\;
    }

    \If{$\mathcal{D}(\hat{P}_n, \hat{P}_\mathcal{B}) \leq \delta$}{
        \Return $n$\;
    }
}
\Return $\mathcal{B}$\;
\end{algorithm}

Algorithm~\ref{alg:aposteriori} takes as input:
\begin{itemize}
\item A list of measurement outcomes ${x_1, x_2, \dots, x_\mathcal{B}}$,
\item A maximum estimation error threshold $\delta > 0$,
\item A divergence metric $\mathcal{D}(\cdot, \cdot)$ to compare discrete probability distributions.
\end{itemize}
The output is the smallest number of samples $n^* \leq \mathcal{B}$ such that the empirical distribution $\hat{P}_n$ obtained from the first $n$ samples is within $\delta$ of the full empirical distribution $\hat{P}_\mathcal{B}$.

To perform this task, the algorithm maintains two dictionaries (or \textit{maps}), mapping outcomes $k$ to their frequency counts:
\begin{itemize}
\item \texttt{count\_B}: a dictionary of all outcomes in the full batch, used to compute the reference distribution $\hat{P}_\mathcal{B}$.
\item \texttt{count\_n}: a dictionary of outcomes encountered up to step $n$, used to compute the prefix distribution $\hat{P}_n$.
\end{itemize}

\noindent
The algorithm proceeds in two main steps:
\begin{enumerate}
\item In the first step, the algorithm builds the full empirical distribution $\hat{P}_\mathcal{B}$ from all $\mathcal{B}$ samples. The dictionary \texttt{count\_B} is populated by incrementing counts for each outcome $x_i$. Then, $\hat{P}_\mathcal{B}$ is obtained by normalising these counts over $\mathcal{B}$.
\item In the second step, the algorithm iteratively builds the empirical distribution $\hat{P}_n$ using the first $n$ samples. For each value of $n$ from $1$ to $\mathcal{B}$, it:
\begin{itemize}
    \item Updates \texttt{count\_n} with the $n$-th outcome $x_n$.
    \item Computes the distribution $\hat{P}_n$ by normalizing \texttt{count\_n} over \texttt{total\_n}.
    \item Computes the divergence $\mathcal{D}(\hat{P}_n, \hat{P}_\mathcal{B})$.
\end{itemize}
If the divergence is less than or equal to $\delta$, the algorithm returns $n$ as the optimal shot count $n^*$.

\item If no such $n$ is found before reaching $\mathcal{B}$, the algorithm defaults to returning $\mathcal{B}$.
\end{enumerate}

This procedure is not usable online, as it requires all $\mathcal{B}$ outcomes to compute the reference distribution $\hat{P}_\mathcal{B}$. However, it serves as a retrospective baseline for evaluating the efficiency of sample-based estimation strategies and provides a concrete definition of convergence under budget constraints.

\subsection{The Point of Diminishing Returns as a Practical Approximation}
\label{sec:info-conv}

% Considering the aim to determining $n^*$ \textit{during} the sampling process and not \textit{a posteriori}, we introduce the concept of \textit{information convergence} to recognize when $\hat{P}_n$ is enough \textit{close} to $\hat{P}_\mathcal{B}$.

To enable \textit{online}, data-driven decision making in the absence of the ground truth distribution $P$, we introduce the concept of \emph{the point of diminishing returns} as a practical, assumption-free proxy for accuracy. The core idea is to monitor how much the empirical distribution changes as more samples are collected. When this change becomes negligible, the distribution can be considered statistically stable, and further sampling may be unnecessary.

\begin{definition}[\textbf{Approximate Point of Diminishing Returns}]
\label{def:info-conv}
Let $\hat{P}_n$ be the cumulative empirical distribution after $n \leq \mathcal{B}$ samples, and let $ \mathcal{D}(\cdot,\cdot)$ be a divergence metric over distributions. Given a look-back window $\tau$, the \textit{approximate} point of diminishing returns is said to occur at step $n$ if $n$ is the smallest value such that:
\[
\mathcal{D}\left( \hat{P}_n, \hat{P}_{n - \tau} \right) \leq \varepsilon
\]
where $\varepsilon > 0$ is a tolerance parameter controlling sensitivity to change.
\end{definition}

Since the accuracy threshold $\delta$ is linked to the knowledge of the empirical distribution $\hat{P_{\mathcal{B}}}$, our notion of approximate point of diminishing returns relies on a $\varepsilon$ threshold which acts as the $\delta$ threshold but in an online fashion. Depending on the actual scenario, they can be the same or differ. In our \textsc{IncrementalExecution} Framework $\varepsilon$ is an hyperparameter.

While this does not guarantee closeness to the true distribution $P$, it provides an observable indication that the output distribution $\hat{P}_n$ is stabilising. Experiments (Sect.~\ref{sec:exp}) will prove that the approximate point of diminishing returns acts as a practical, online approximation of the a posteriori optimality criterion defined in Definition~\ref{def:optimal-shots}.

\subsection{The Quantum Black-box Shot Optimisation Problem}
\label{sec:quantum-problem}

% The \textit{Black-box Shot Optimisation Problem} (Definition~\ref{def:problem}) finds a compelling instantiation in quantum computing, where sampling corresponds to performing shots of a quantum circuit on a (noisy) quantum processing unit (QPU). Each shot yields a single measurement outcome from one execution of the circuit, and the collection of these outcomes approximates the circuit’s output distribution under realistic, noise-affected conditions.

% Formally, let $C$ denote a quantum circuit. When executed on an ideal, noiseless quantum simulator, $C$ induces a target distribution $P_C$ over its possible measurement outcomes, i.e., our \textit{ground-truth}. However, when run on a real Q, stochastic noise alters the circuit’s execution, yielding an unknown distribution $P(C, Q)$. Since we make no assumptions about the internal noise model of the Q or the structure of $C$, we treat the system as a black-box sampler from the effective output distribution $P = P(C, Q)$.

% In this black-box setting, the true distribution $P = P(C, Q)$ remains unknown. We must instead rely on empirical distributions $\hat{P}_n$ formed by aggregating the outcomes of $n$ circuit executions (shots). Given a maximum budget of $\mathcal{B}$ shots, the empirical distribution $\hat{P}_\mathcal{B}$ serves as the best attainable estimate of $P$ under the budget constraints.

The \textit{Black-box Sample Optimisation Problem} (Definition~\ref{def:problem}) finds a compelling instantiation in the context of quantum computing. Executing a shot of a quantum circuit is analogous to drawing a sample from an unknown probability distribution $P$. Similarly, performing $n$ shots corresponds to generating an empirical distribution $\hat{P}_n$. The budget $\mathcal{B}$ represents the maximum amount of shots allowed.

In the quantum computing scenario, our objective is to determine the minimal number of shots $n^*$ required to reduce the divergence between $\hat{P}_n$ and $P$. In other words, to find the smallest sample size that sufficiently approximates the unknown distribution $P$.

This task is complicated by the fact that, in practice, quantum circuits are executed on noisy QPUs. Each shot produces a single measurement outcome from one execution of the circuit, and the aggregation of these outcomes forms an approximation of the circuit's output distribution under realistic, noise-affected conditions. For those reasons, executing a quantum circuit $C$ on a quantum computer $Q$ produce a noisy distribution denoted by $P(C, Q)$, which can empirically sampled through $n$ shots, resulting in $\hat{P}(C, Q)_n$.

Consequently, we define the black-box sample optimisation problem in the quantum setting as follows:

\begin{definition}[\textbf{The Quantum Black-box Shot Optimisation Problem}]
\label{def:quantum-problem}
Given a quantum circuit $C$ and a noisy quantum process unit $Q$, and a maximum shot budget $\mathcal{B} \in \mathbb{N}$, determine the smallest natural number $n^* \leq \mathcal{B}$ such that:
\[
n^* = \min \left\{ n \leq \mathcal{B} \mid \mathcal{D}(\hat{P}(C,Q)_n, \hat{P}(C,Q)_\mathcal{B}) \leq \delta \right\},
\]


where $\hat{P}(C, Q)_n$ denotes the empirical distribution obtained by performing $n$ shots of $C$ on $Q$; $\hat{P}(C, Q)_\mathcal{B}$ denotes the empirical distribution obtained using the full budget $\mathcal{B}$; and $\delta > 0$ is the tolerance threshold below which $\hat{P}(C, Q)_n$ is considered a sufficiently accurate approximation of $\hat{P}(C, Q)_\mathcal{B}$, thus reaching the point of diminishing returns.
\end{definition}

Since $\hat{P}(C, Q)_\mathcal{B}$ represents the best approximation to $P(C, Q)$ obtainable with the shot budget, finding an optimal $n^* \leq \mathcal{B}$ enables saving the cost of $\mathcal{B} - n^*$ shots, while achieving similar empirical accuracy as $\hat{P}(C, Q)_\mathcal{B}$.

From this point forward, we adopt the Total Variation Distance (TVD) as our distance metric $\mathcal{D}$ and we apply it to quantify the difference between distributions. Given two discrete probability distributions $P$ and $P'$ over the same outcome space $\mathcal{X}$, the Total Variation Distance is defined as:
\[
\mathrm{TVD}(P, P') = \frac{1}{2} \sum_{x \in \mathcal{X}} \left| P(x) - P'(x) \right|.
\]
This metric has a natural interpretation: it corresponds to the maximum discrepancy in probability mass that the two distributions assign to the same event, and ranges from 0 (identical distributions) to 1 (disjoint support). We selected TVD for its simplicity, interpretability, and widespread use in statistical and quantum information theory contexts.

\begin{figure*}[t]
\centering
\subfigure[TVD to ideal distribution as a function of shot count.]{\includegraphics[width=0.49\textwidth]{img/distancetvd.png}}
\hfill
\subfigure[Change in empirical distribution between successive windows ($\tau=50$).]{\includegraphics[width=0.49\textwidth]{img/deltatvd.png}}
\caption{Empirical behaviour of quantum circuit output distributions as shots increase. Each line represents a unique circuit-backend pair.}
\Description{Two line plots. The first shows the Total Variation Distance (TVD) between the empirical and ideal distributions as a function of the number of shots for multiple circuit-backend pairs; TVD decreases and stabilises over time. The second shows the divergence between consecutive empirical distributions (Delta-TVD) over a sliding window of size 50; all lines show a rapid decay and plateau, indicating convergence.}
\label{fig:tvd}
\end{figure*}

\subsection*{Preliminary Study}
To assess the feasibility and soundness of our approach, we conducted a preliminary study aimed at evaluating whether output distributions exhibit stabilisation and convergence as the number of shots increases. We also investigated whether this behaviour, if observed, can be effectively captured by our proposed definition of approximate point of diminishing returns. 

Figure~\ref{fig:tvd} presents empirical evidence of these dynamics. Each line corresponds to a unique pair consisting of a quantum circuit and a noisy quantum backend. We considered 28 different circuits with qubit counts ranging from 4 to 16 and executed them on five IBM noisy simulators. For each circuit-backend pair, we ran the circuit in batches of $\tau = 50$ shots, up to a total of $\mathcal{B}=20{,}000$ samples, recording the empirical distribution $\hat{P}_n$ after each batch.


In subfigure~(a), we compute the Total Variation Distance (TVD) between each empirical distribution $\hat{P}_n$ and the corresponding ideal distribution $P_C$, obtained by executing the same circuit on a perfect noiseless simulator. When the number of shots is low, the TVD is unstable due to the high variance inherent in small-sample estimates, which can lead to significant deviations from the true distribution purely by chance. As the number of shots increases, the empirical distribution becomes a more accurate approximation of the underlying probability distribution, reducing statistical fluctuations. Consequently, the TVD decreases, reflecting improved estimation accuracy. Eventually, the TVD plateaus, indicating that further increasing the number of shots yields only marginal gains, as the estimation error becomes dominated by systematic effects such as hardware noise rather than sampling noise.

Subfigure~(b) shows the \emph{Delta-TVD} -- that is, the divergence between successive empirical distributions computed over a fixed sliding window of size $\tau = 50$. For each pair, we measure the change between $\hat{P}_n$ and $\hat{P}_{n-\tau}$ using TVD. The initial rapid drop followed by a plateau indicates that the output distribution stabilises over time, reaching the \textit{point of diminishing returns} as defined in Section~\ref{sec:info-conv}.

\paragraph{Advantages in Quantum Contexts.} The approximate point of diminishing returns provides a practical and flexible convergence signal in quantum computing:
\begin{itemize}
\item It does not rely on the circuit’s structure, noise model, or ideal distribution $P_C$, making it applicable across diverse quantum computer architectures and circuit types.
\item It can be computed online, requiring only a running history of observed outputs and not the true distribution.
\item It naturally adapts to circuit- and backend-specific behaviour, supporting dynamic shot allocation tailored to the circuit’s statistical complexity.
\item It is metric-agnostic and can be used with various divergence measures, such as TVD, Jensen–Shannon divergence, or Hellinger distance.
\end{itemize}

In summary, the quantum black-box setting offers a concrete real-world instantiation of the \textit{Black-box Sample Optimisation Problem}. The concept of point of diminishing returns enables an online, adaptive stopping rule for quantum circuit execution, offering a principled foundation for general-purpose shot management strategies. In the next section, we build on this foundation to introduce the \textsc{IncrementalExecution} framework, which implements these ideas as a fully online optimisation procedure for shot allocation in quantum experiments.
